KGARevion: An AI Agent for Knowledge-Intensive Biomedical QA

Biomedical reasoning integrates structured, codified knowledge with tacit, experience-driven insights. Depending on the context, quantity, and nature of available evidence, researchers and clinicians use diverse strategies, including rule-based, prototype-based, and case-based reasoning. Effective medical AI models must handle this complexity while ensuring reliability and adaptability. We introduce KGARevion, a knowledge graph-based agent that answers knowledge-intensive questions. Upon receiving a query, KGARevion generates relevant triplets by leveraging the latent knowledge embedded in a large language model. It then verifies these triplets against a grounded knowledge graph, filtering out errors and retaining only accurate, contextually relevant information for the final answer. This multi-step process strengthens reasoning, adapts to different models of medical inference, and outperforms retrieval-augmented generation-based approaches that lack effective verification mechanisms. Evaluations on medical QA benchmarks show that KGARevion improves accuracy by over 5.2% over 15 models in handling complex medical queries. To further assess its effectiveness, we curated three new medical QA datasets with varying levels of semantic complexity, where KGARevion improved accuracy by 10.4%. The agent integrates with different LLMs and biomedical knowledge graphs for broad applicability across knowledge-intensive tasks. We evaluated KGARevion on AfriMed-QA, a newly introduced dataset focused on African healthcare, demonstrating its strong zero-shot generalization to underrepresented medical contexts.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> table.tex <==
\begin{table*}[h!t]
\caption{The accuracy of \model and all baselines on four gold standard and three newly created datasets under multi-choice reasoning settings. The value highlighted in \colorbox{NavyBlue!10}{Blue} indicates the best result among LLM-based reasoning models with a size smaller than 8B, including LLaMA3-8B, while \colorbox{Red!30}{Red} marks the top value among LLaMA3.1-8B and other types of baselines. std means the standard deviation under three runs.}
\vspace{1mm}
\centering
\resizebox{1\columnwidth}{!}{
	\begin{tabular}{lcccc|ccc}
		\toprule
            \multirow{1}{*}{\textbf{Multi-choice Reasoning}} & \multicolumn{4}{c}{Established Medical QA Benchmarks} & \multicolumn{3}{c}{MedDDx}\\
            \cmidrule(r){2-5} \cmidrule(r){6-8}
            \multirow{1}{*}{Method}
            & MMLU-Med & MedQA-US & PubMedQA* & BioASQ-Y/N  & Basic & Intermediate & Expert\\
            \midrule  
            %\multicolumn{8}{c}{LLM-based Reasoning Models}\\
            Metrics &  Acc. (std) &    Acc. (std)&    Acc. (std)&    Acc. (std)&    Acc. (std)&    Acc. (std)&    Acc. (std)  \\
            \hline
            %\hline
            \rowcolor{NavyBlue!10}LLaMA2-7B & 0.376 \footnotesize{(.006)}  &  0.281 \footnotesize{(.004)}  &  0.448 \footnotesize{(.010)}  & 0.568 \footnotesize{(.006)} & 0.215 \footnotesize{(.030)} &  0.198 \footnotesize{(.004)}  &  0.192 \footnotesize{(.012)} \\
            \rowcolor{NavyBlue!10}LLaMA2-7B (CoT) &   0.318 \footnotesize{(.005)} &   0.251 \footnotesize{(.002)} &  0.465 \footnotesize{(.011)} &   0.547 \footnotesize{(.011)} &  0.289 \footnotesize{(.010)} &   0.265 \footnotesize{(.006)} &   0.229 \footnotesize{(.023)} \\

            \rowcolor{NavyBlue!10}Mistral-7B & 0.634 \footnotesize{(.004)}  & 0.477 \footnotesize{(.007)} & 0.400 \footnotesize{(.002)}  & 0.644 \footnotesize{(.001)} & 0.412 \footnotesize{(.003)}&   0.356 \footnotesize{(.003)}  &  0.375 \footnotesize{(.007)}\\
            \rowcolor{NavyBlue!10}Mistral-7B  (CoT) & 0.634 \footnotesize{(.003)} &  0.474 \footnotesize{(.002)} &  0.372 \footnotesize{(.005)} &   0.651 \footnotesize{(.002)} & 0.404 \footnotesize{(.010)} &  0.368 \footnotesize{(.023)} &  \textbf{\textcolor{NavyBlue}{0.379}} \footnotesize{\textcolor{NavyBlue}{(.027)}} \\
            
            \rowcolor{NavyBlue!10}MedAlpaca-7B  &  0.600 \footnotesize{(.004)}  &  0.401 \footnotesize{(.001)}  &  0.333 \footnotesize{(.015)}  &  0.493 \footnotesize{(.034)} & 0.399 \footnotesize{(.012)} &  0.325 \footnotesize{(.004)}  &  0.311 \footnotesize{(.009)} \\
            \rowcolor{NavyBlue!10}MedAlpaca-7B  (CoT)  &   0.603 \footnotesize{(.004)} &   0.399 \footnotesize{(.003)} &   0.315 \footnotesize{(.015)} &   0.485 \footnotesize{(.025)} & 0.395 \footnotesize{(.007)} &   0.321 \footnotesize{(.011)} &   0.312 \footnotesize{(.010)} \\

            \rowcolor{NavyBlue!10}PMC-LLaMA-7B &  0.207 \footnotesize{(.011)} &  0.247 \footnotesize{(.004)}  &  0.179 \footnotesize{(.007)}  &  0.346 \footnotesize{(.017)}  & 0.087 \footnotesize{(.015)} &  0.086 \footnotesize{(.002)} &  0.079 \footnotesize{(.006)}  \\
            \rowcolor{NavyBlue!10}PMC-LLaMA-7B  (CoT)&  0.204 \footnotesize{(.008)} &   0.208 \footnotesize{(.002)} &   0.125 \footnotesize{(.014)} &  0.208 \footnotesize{(.002)} &  0.088 \footnotesize{(.002)} &  0.077 \footnotesize{(.004)} &  0.063 \footnotesize{(.005)} \\

            %\cline{1-8}
            
            \rowcolor{NavyBlue!10}LLaMA3-8B  & 0.634 \footnotesize{(.005)}  &  \textbf{\textcolor{NavyBlue}{0.566}} \footnotesize{\textcolor{NavyBlue}{(.004)}} &  \textbf{\textcolor{NavyBlue}{0.586}} \footnotesize{\textcolor{NavyBlue}{(.008)}}  & 0.654  \footnotesize{(.005)}  &  0.428 \footnotesize{(.015)}  &  0.319 \footnotesize{(.002)} &  0.306 \footnotesize{(.009)} \\
            \rowcolor{NavyBlue!10}LLaMA3-8B (CoT) &  \textbf{\textcolor{NavyBlue}{0.651}} \footnotesize{\textcolor{NavyBlue}{(.003)}} &  0.552 \footnotesize{(.003)}& 0.574 \footnotesize{(.002)} &  \textbf{\textcolor{NavyBlue}{0.681}} \footnotesize{\textcolor{NavyBlue}{(.002)}}  &   \textbf{\textcolor{NavyBlue}{0.434}} \footnotesize{\textcolor{NavyBlue}{(.010)}} &  \textbf{\textcolor{NavyBlue}{0.368}} \footnotesize{\textcolor{NavyBlue}{(.004)}} &  0.313 \footnotesize{(.003)} \\

            \rowcolor{NavyBlue!10}Llama3-OpenBioLLM-8B &  0.636 \footnotesize{(.005)}  & 0.383 \footnotesize{(.003)}  & 0.350 \footnotesize{(.026)}  & 0.623 \footnotesize{(.005)} & 0.238 \footnotesize{(.004)} &  0.235 \footnotesize{(.011)}&  0.229 \footnotesize{(.020)}  \\
            \rowcolor{NavyBlue!10}Llama3-OpenBioLLM-8B (CoT)&   0.571 \footnotesize{(.003)} &  0.295 \footnotesize{(.002)} &   0.283 \footnotesize{(.001)} &  0.646 \footnotesize{(.004)} &  0.370 \footnotesize{(.013)} &  0.330 \footnotesize{(.001)} &  0.327 \footnotesize{(.011)}  \\

            \hline
            \rowcolor{Red!10}LLaMA3.1-8B & 0.677 \footnotesize{(.007)}  & \textbf{\textcolor{Red}{0.563}} \footnotesize{\textcolor{Red}{(.006)}}  & 0.596 \footnotesize{(.009)} & 0.687 \footnotesize{(.006)} & 0.434 \footnotesize{(.018)} &  0.368 \footnotesize{(.002)} &  0.306 \footnotesize{(.021)} \\
            \rowcolor{Red!10}LLaMA3.1-8B (CoT) &  \textbf{\textcolor{Red}{0.681}} \footnotesize{\textcolor{Red}{(.005)}} &   0.549 \footnotesize{(.003)} &   \textbf{\textcolor{Red}{0.600}} \footnotesize{\textcolor{Red}{(.005)}} &  0.706 \footnotesize{(.002)}&  \textbf{\textcolor{Red}{0.439}} \footnotesize{\textcolor{Red}{(.017)}} &  0.393 \footnotesize{(.005)} &  0.322 \footnotesize{(.014)} \\
            
            \rowcolor{Red!10}LLaMA2-13B  & 0.442 \footnotesize{(.002)}  & 0.253 \footnotesize{(.004)}  & 0.252 \footnotesize{(.004)}  & 0.455 \footnotesize{(.002)}  &   0.286 \footnotesize{(.003)}  &    0.338 \footnotesize{(.006)}  &    0.317 \footnotesize{(.006)}  \\
            \rowcolor{Red!10}LLaMA2-13B (CoT) &   0.415 \footnotesize{(.002)} &   0.354 \footnotesize{(.005)} &  0.232 \footnotesize{(.006)} &  0.422 \footnotesize{(.003)} &   0.309 \footnotesize{(.005)} &    0.263 \footnotesize{(.013)} &   0.243 \footnotesize{(.016)} \\
            
            \hline\hline
            
            \rowcolor{Red!10}QAGNN & 0.317 \footnotesize{(.003)} & 0.450 \footnotesize{(.005)} & 0.439 \footnotesize{(.033)} & 0.644 \footnotesize{(.002)}  &  0.295 \footnotesize{(.003)} & 0.265 \footnotesize{(.002)} & 0.253 \footnotesize{(.003)} \\
            \rowcolor{Red!10}JointLK & 0.288 \footnotesize{(.005)} & 0.472 \footnotesize{(.003)} & 0.468 \footnotesize{(.007)} & 0.640 \footnotesize{(.007)} &  0.247 \footnotesize{(.004)} & 0.250 \footnotesize{(.003)} & 0.244 \footnotesize{(.004)} \\
            \rowcolor{Red!10}Dragon & 0.319 \footnotesize{(.003)} & 0.475 \footnotesize{(.002)} & 0.472 \footnotesize{(.005)} &  0.646 \footnotesize{(.003)} & 0.286 \footnotesize{(.003)} & 0.247 \footnotesize{(.005)} & 0.240 \footnotesize{(.004)} \\
            
            \hline\hline
            
            \rowcolor{Red!10}Self-RAG (7B) & 0.322 \footnotesize{(.019)} & 0.380 \footnotesize{(.028)} & 0.534 \footnotesize{(.028)} & 0.594 \footnotesize{(.012)} &   0.238 \footnotesize{(.007)} & 0.199 \footnotesize{(.037)} & 0.224 \footnotesize{(.045)} \\
            \rowcolor{Red!10}Self-RAG (13B) & 0.502 \footnotesize{(.004)} & 0.408 \footnotesize{(.020)} & 0.331 \footnotesize{(.158)} & 0.646 \footnotesize{(.050)} &  0.249 \footnotesize{(.010)} & 0.290 \footnotesize{(.018)} & 0.266 \footnotesize{(.031)}\\
            \rowcolor{Red!10}KG-Rank (13B) & 0.452 \footnotesize{(.005)} & 0.362 \footnotesize{(.011)} & 0.305 \footnotesize{(.019)} & 0.503 \footnotesize{(.015)} & 0.253 \footnotesize{(.021)} & 0.256 \footnotesize{(.013)} & 0.234 \footnotesize{(.010)}  \\
            \rowcolor{Red!10}KG-RAG (8B) & 0.516 \footnotesize{(.005)} & 0.343 \footnotesize{(.001)} & 0.429 \footnotesize{(.017)} & 0.662 \footnotesize{(.005)} &  0.434 \footnotesize{(.021)} & \textbf{\textcolor{Red}{0.413}} \footnotesize{\textcolor{Red}{(.007)}} & \textbf{\textcolor{Red}{0.391}} \footnotesize{\textcolor{Red}{(.004)}}  \\
            \rowcolor{Red!10}MedRAG (70B) & 0.579 \footnotesize{(.015)} & 0.487 \footnotesize{(.014)} & 0.574 \footnotesize{(.022)} & \textbf{\textcolor{Red}{0.719}} \footnotesize{\textcolor{Red}{(.018)}} & 0.365 \footnotesize{(.008)} & 0.348 \footnotesize{(.011)} & 0.327 \footnotesize{(.003)} \\
            \hline\hline
             \rowcolor{NavyBlue!10}\model (LLaMA3, w/o Review) & 0.621 \footnotesize{(.002)}  &  0.528 \footnotesize{(.003)}  & 0.556 \footnotesize{(.002)}  & 0.713 \footnotesize{(.004)} & 0.310 \footnotesize{(.006)} & 0.334 \footnotesize{(.004)}  & 0.313 \footnotesize{(.008)} \\
            \rowcolor{NavyBlue!10}\model (LLaMA3, w/o Revise) & 0.657 \footnotesize{(.004)}  &  0.594 \footnotesize{(.006)}  &  0.562 \footnotesize{(.002)}  & 0.723 \footnotesize{(.005)} & 0.386 \footnotesize{(.008)} & 0.372 \footnotesize{(.004)}  & 0.327 \footnotesize{(.003)} \\
            \rowcolor{NavyBlue!10}\model (LLaMA3, $k = 1$) &  \textbf{\textcolor{NavyBlue}{0.703}} \footnotesize{\textcolor{NavyBlue}{(.004)}} & 0.610 \footnotesize{(.010)} & 0.562 \footnotesize{(.002)} & \textbf{\textcolor{NavyBlue}{0.744}} \footnotesize{(.003)} & \textbf{\textcolor{NavyBlue}{0.473}} \footnotesize{\textcolor{NavyBlue}{(.008)}} & 0.404 \footnotesize{(.006)} & 0.395 \footnotesize{(.003)}\\
            \rowcolor{NavyBlue!10}\model (LLaMA3, $k = 2$) & 0.696 \footnotesize{(.006)}  &  0.616 \footnotesize{(.008)}  &  0.566 \footnotesize{(.002)} & 0.723 \footnotesize{(.010)} & 0.457 \footnotesize{(.006)} & 0.414 \footnotesize{(.006)} & 0.395 \footnotesize{(.005)} \\
            \rowcolor{NavyBlue!10}\model (LLaMA3, $k = 3$) & 0.678 \footnotesize{(.006)}  & \textbf{\textcolor{NavyBlue}{0.628}} \textcolor{NavyBlue}{\footnotesize{(.002)}}  & \textbf{\textcolor{NavyBlue}{0.590}} \textcolor{NavyBlue}{\footnotesize{(.005)}}  & 0.737 \footnotesize{(.007)}  & 0.469 \footnotesize{(.008)} & \textbf{\textcolor{NavyBlue}{0.451}} \textcolor{NavyBlue}{\footnotesize{(.004)}}  & \textbf{\textcolor{NavyBlue}{0.411}} \footnotesize{\textcolor{NavyBlue}{(.005)}} \\
            \textbf{\textcolor{NavyBlue}{Improvement over best baseline}} & \textbf{\textcolor{NavyBlue}{+5.2\%}}  &  \textbf{\textcolor{NavyBlue}{+6.2\%}} & \textbf{\textcolor{NavyBlue}{+0.4\%}}  & \textbf{\textcolor{NavyBlue}{+6.3\%}}  & \textbf{\textcolor{NavyBlue}{+3.9\%}} & \textbf{\textcolor{NavyBlue}{+8.3\%}}  & \textbf{\textcolor{NavyBlue}{+3.2\%}}\\ 
            \midrule
            \rowcolor{Red!10}\model (LLaMA3.1, w/o Review) &  0.695 \footnotesize{(.006)} &  0.546 \footnotesize{(.002)}  &  0.560 \footnotesize{(.004)}  & 0.736 \footnotesize{(.003)} & 0.298 \footnotesize{(.015)} & 0.299 \footnotesize{(.003)} & 0.327 \footnotesize{(.006)}  \\
            \rowcolor{Red!10}\model (LLaMA3.1, w/o Revise) &  0.716 \footnotesize{(.006)}  & 0.573 \footnotesize{(.005)}  &  0.568 \footnotesize{(.011)} &  0.749 \footnotesize{(.003)} &  0.392 \footnotesize{(.012)} & 0.337 \footnotesize{(.006)}  & 0.352 \footnotesize{(.005)} \\
            \rowcolor{Red!10}\model (LLaMA3.1, $k = 1$) & \textbf{\textcolor{Red}{0.734}} \footnotesize{\textcolor{Red}{(.004)}} & 0.618 \footnotesize{(.002)} &  0.619 \footnotesize{(.004)} & \textbf{\textcolor{Red}{0.763}} \footnotesize{(.001)} & \textbf{\textcolor{Red}{0.483}} \footnotesize{\textcolor{Red}{(.013)}} & \textbf{\textcolor{Red}{0.457}} \footnotesize{\textcolor{Red}{(.010)}}& 0.409 \footnotesize{(.005)}\\
            \rowcolor{Red!10}\model (LLaMA3.1, $k = 2$) &  0.720 \footnotesize{(.003)} &  0.616 \footnotesize{(.005)}  & 0.656 \footnotesize{(.006)}  & 0.745 \footnotesize{(.005)}  & 0.396 \footnotesize{(.003)} & 0.454 \footnotesize{(.008)}  & 0.342 \footnotesize{(.004)} \\
            \rowcolor{Red!10}\model (LLaMA3.1, $k = 3$) & 0.716 \footnotesize{(.004)}  & \textbf{\textcolor{Red}{0.620}} \textcolor{red}{\footnotesize{(.003)}}  &  \textbf{\textcolor{Red}{0.638}} \textcolor{red}{\footnotesize{(.004)}} & 0.749 \footnotesize{(.003)} & 0.469 \footnotesize{(.012)} & 0.411 \footnotesize{(.010)}  & \textbf{\textcolor{Red}{0.447}} \footnotesize{\textcolor{Red}{(.005)}} \\
            \textbf{\textcolor{Red}{Improvement over best baseline}} & \textbf{\textcolor{Red}{+5.3\%}}  & \textbf{\textcolor{Red}{+5.7\%}}  & \textbf{\textcolor{Red}{+3.8\%}}  & \textbf{\textcolor{Red}{+4.4\%}}  & \textbf{\textcolor{Red}{+4.4\%}} & \textbf{\textcolor{Red}{+4.4\%}}  & \textbf{\textcolor{Red}{+5.6\%}}\\ 
            \toprule
	\end{tabular}
 }
\label{main_results}
\vspace{-6mm}
\end{table*}

\subsection{Benchmarking \model under \underline{Open-ended Reasoning Setting}}
\begin{figure}[!t]
    \centering
    \includegraphics[width=1.05\linewidth]{FIG/medical_concepts.pdf}
    \caption{The accuracy of \model and pure LLMs with the medical concepts increase under {\textbf a)} multi-choice reasoning setting and {\textbf b)} open-ended reasoning setting.}
    \label{fig:concepts}
    \vspace{-3mm}
\end{figure}

\begin{table*}[t]
\caption{The accuracy of \model and baselines on four gold standard and three newly created datasets under open-ended reasoning settings. The value highlighted in \colorbox{NavyBlue!10}{Blue} indicates the best result among LLM-based reasoning models with a size smaller than 8B, including LLaMA3-8B, while \colorbox{Red!30}{Red} marks the top value among LLaMA3.1-8B and other types of baselines. $\Delta$Acc. denotes the difference in performance between the open-ended and multiple-choice reasoning settings.}
\vspace{1mm}
\centering
\resizebox{1\columnwidth}{!}{
	\begin{tabular}{lcccc|ccc}
		\toprule
            \multirow{1}{*}{\textbf{Open-ended Reasoning}} & \multicolumn{4}{c}{\textbf{Open-ended inquiries without pre-defined choices}} & \multicolumn{3}{c}{MedDDx-No-Opt} (\textbf{Open-ended})\\
            \cmidrule(r){2-5} \cmidrule(r){6-8}
            \multirow{1}{*}{Method}
            & MMLU-Med & MedQA-US & PubMedQA* & BioASQ-Y/N  & Basic & Intermediate & Expert\\
            \midrule  
            %\multicolumn{8}{c}{LLM-based Reasoning Models}\\
            Metrics &  Acc. $\Delta$Acc. &  Acc. $\Delta$Acc.&  Acc. $\Delta$Acc.&  Acc. $\Delta$Acc.&  Acc. $\Delta$Acc.&  Acc. $\Delta$Acc.&  Acc. $\Delta$Acc.  \\
            \hline
           \rowcolor{NavyBlue!10} LLaMA2-7B &  0.328 \footnotesize{(-0.048)} &  0.302 \footnotesize{(+0.021)}  &  0.546 \footnotesize{(+0.098)}  &  0.625 \footnotesize{(+0.057)}  &  0.286 \footnotesize{(+0.071)} &  0.305 \footnotesize{(+0.107)} & 0.302 \footnotesize{(+0.110)} \\
            \rowcolor{NavyBlue!10}LLaMA2-7B (CoT)  & 0.362 \footnotesize{(+0.044)}  &  0.243 \footnotesize{(-0.008)}  &  0.418 \footnotesize{(-0.047)}  & 0.642 \footnotesize{(+0.095)} &  0.265 \footnotesize{(-0.024)} & 0.270 \footnotesize{(+0.005)} & 0.280 \footnotesize{(+0.051)} \\

            \rowcolor{NavyBlue!10}Mistral-7B  &  0.591 \footnotesize{(-0.043)} & 0.412 \footnotesize{(-0.065)} &  0.344 \footnotesize{(-0.056)}  & 0.629 \footnotesize{(-0.015)}  & 0.249 \footnotesize{(-0.163)} & 0.228 \footnotesize{(-0.128)} & 0.273 \footnotesize{(-0.102)} \\
            \rowcolor{NavyBlue!10}Mistral-7B  (CoT)  & 0.583 \footnotesize{(-0.051)}  &  0.398 \footnotesize{(-0.076)}  &  0.212 \footnotesize{(-0.160)}  & 0.657 \footnotesize{(+0.006)}  & 0.245 \footnotesize{(-0.159)} & 0.232 \footnotesize{(-0.136)}  & 0.286 \footnotesize{(-0.093)} \\

            \rowcolor{NavyBlue!10}PMC-LLaMA-7B  & 0.073 \footnotesize{(-0.134)}  &  0.082 \footnotesize{(-0.165)}  &  0.090 \footnotesize{(-0.089)}  &  0.139 \footnotesize{(-0.201)} & 0.249 \footnotesize{(+0.162)} & 0.191 \footnotesize{(+0.105)} & 0.232 \footnotesize{(+0.153)}  \\
            \rowcolor{NavyBlue!10}PMC-LLaMA-7B  (CoT) &  0.080 \footnotesize{(-0.124)} &  0.079 \footnotesize{(-0.129)}  &  0.092 \footnotesize{(-0.033)}  & 0.125 \footnotesize{(-0.083)}  & 0.220 \footnotesize{(+0.132)} & 0.245 \footnotesize{(+0.168)}  & 0.228 \footnotesize{(+0.165)} \\
            %\cline{1-8}
            
            \rowcolor{NavyBlue!10}LLaMA3-8B   & 0.595 \footnotesize{(-0.039)}  &  \textbf{\textcolor{NavyBlue}{0.458}} \footnotesize{\textcolor{NavyBlue}{(-0.108)}}  &  0.532 \footnotesize{(-0.054)}  & 0.672 \footnotesize{(+0.018)}  & \textbf{\textcolor{NavyBlue}{0.343}} \footnotesize{\textcolor{NavyBlue}{(-0.085)}} & \textbf{\textcolor{NavyBlue}{0.314}} \footnotesize{\textcolor{NavyBlue}{(-0.005)}}  & 0.317 \footnotesize{(+0.011)} \\
            \rowcolor{NavyBlue!10}LLaMA3-8B (CoT) & \textbf{\textcolor{NavyBlue}{0.608}} \footnotesize{\textcolor{NavyBlue}{(-0.043)}}  &  0.449 \footnotesize{(-0.103)}  & \textbf{\textcolor{NavyBlue}{0.562}} \footnotesize{\textcolor{NavyBlue}{(-0.012)}}  & \textbf{\textcolor{NavyBlue}{0.714}} \footnotesize{\textcolor{NavyBlue}{(+0.033)}} & 0.289 \footnotesize{(-0.145)}& 0.304 \footnotesize{(-0.064)} & \textbf{\textcolor{NavyBlue}{0.327}} \footnotesize{\textcolor{NavyBlue}{(+0.014)}}\\

            \rowcolor{NavyBlue!10}Llama3-OpenBioLLM-8B  & 0.324 \footnotesize{(-0.312)} &  0.157 \footnotesize{(-0.226)}  &  0.157 \footnotesize{(-0.193)}  & 0.324 \footnotesize{(-0.299)}  & 0.016 \footnotesize{(-0.222)}  & 0.006 \footnotesize{(-0.229)}  & 0.008 \footnotesize{(-0.221)} \\
            \rowcolor{NavyBlue!10}Llama3-OpenBioLLM-8B (CoT) & 0.398 \footnotesize{(-0.173)}  &  0.146 \footnotesize{(-0.149)}  &  0.100 \footnotesize{(-0.183)}  & 0.142 \footnotesize{(-0.539)}  & 0.098 \footnotesize{(-0.272)} & 0.084 \footnotesize{(-0.246)}  & 0.108 \footnotesize{(-0.219)} \\
            \hline
            \rowcolor{Red!10}LLaMA3.1-8B  & 0.607 \footnotesize{(-0.070)} &  0.551 \footnotesize{(-0.012)}  &  0.514 \footnotesize{(-0.082)}  & 0.694 \footnotesize{(+0.007)}  & \textbf{\textcolor{Red}{0.322}} \footnotesize{\textcolor{Red}{(-0.112)}}  & 0.289 \footnotesize{(-0.079)}  & \textbf{\textcolor{Red}{0.335}} \footnotesize{\textcolor{Red}{(+0.029)}} \\
            \rowcolor{Red!10}LLaMA3.1-8B (CoT)  & \textbf{\textcolor{Red}{0.697}} \footnotesize{\textcolor{Red}{(+0.016)}}  &  \textbf{\textcolor{Red}{0.563}} \footnotesize{\textcolor{Red}{(+0.014)}}  &  \textbf{\textcolor{Red}{0.572}}\footnotesize{\textcolor{Red}{(-0.028)}}  & \textbf{\textcolor{Red}{0.706}} \footnotesize{\textcolor{Red}{(-0.000)}}  & 0.306 \footnotesize{(-0.133)} & \textbf{\textcolor{Red}{0.294}} \footnotesize{\textcolor{Red}{(-0.099)}}  & 0.315 \footnotesize{(-0.007)} \\
            
            \rowcolor{Red!10}LLaMA2-13B   & 0.348 \footnotesize{(-0.094)}  &  0.283 \footnotesize{(+0.030)}  &  0.218 \footnotesize{(-0.034)}  & 0.421 \footnotesize{(-0.034)}  & 0.190 \footnotesize{(-0.096)}  & 0.123 \footnotesize{(-0.215)}  & 0.153 \footnotesize{(-0.164)} \\
            \rowcolor{Red!10}LLaMA2-13B (CoT)  &  0.311 \footnotesize{(-0.104)} &  0.267 \footnotesize{(-0.087)}  &  0.266 \footnotesize{(+0.034)}  &  0.471 \footnotesize{(+0.049)} & 0.269 \footnotesize{(-0.040)}  & 0.268 \footnotesize{(+0.005)}  & 0.282 \footnotesize{(+0.039)} \\
            
            \hline\hline
            
            \rowcolor{Red!10}Self-RAG (7B)  & 0.256 \footnotesize{(-0.066)}  &  0.235 \footnotesize{(-0.145)}  &  0.316 \footnotesize{(-0.218)}  & 0.379 \footnotesize{(-0.215)}  & 0.167 \footnotesize{(-0.071)} & 0.246 \footnotesize{(+0.047)}  & 0.213 \footnotesize{(-0.011)} \\
            \rowcolor{Red!10}Self-RAG (13B)  & 0.309 \footnotesize{(-0.193)}  &  0.297 \footnotesize{(-0.111)}  &  0.438 \footnotesize{(+0.107)}  & 0.539 \footnotesize{(-0.107)} & 0.212 \footnotesize{(-0.037)}  & 0.232 \footnotesize{(-0.058)}  & 0.226 \footnotesize{(--0.040)}  \\
            \rowcolor{Red!10}KG-Rank (13B)  & 0.151 \footnotesize{(-0.301)}  &  0.189 \footnotesize{(-0.173)}  & 0.203 \footnotesize{(-0.102)}  & 0.188 \footnotesize{(-0.315)}  & 0.127 \footnotesize{(-0.126)} & 0.133 \footnotesize{(-0.123)}  & 0.133 \footnotesize{(-0.101)} \\
            \rowcolor{Red!10}KG-RAG (8B)  & 0.310 \footnotesize{(-0.206)}  & 0.290 \footnotesize{(-0.053)}  &  0.316 \footnotesize{(-0.113)}  & 0.359 \footnotesize{(-0.303)}  & 0.216 \footnotesize{(-0.218)} & 0.220 \footnotesize{(-0.193)}  & 0.213 \footnotesize{(-0.178)} \\
            \hline\hline
            \rowcolor{NavyBlue!10}\model (LLaMA3, w/o Review) & 0.645 \footnotesize{(+0.024)}  &  0.609 \footnotesize{(+0.081)}  &  0.552 \footnotesize{(-0.004)}  & 0.701 \footnotesize{(-0.012)}  & 0.400 \footnotesize{(+0.090)} & 0.360 \footnotesize{(+0.026)} & 0.356 \footnotesize{(+0.043)} \\
            \rowcolor{NavyBlue!10}\model (LLaMA3, w/o Revise) &  0.668 \footnotesize{(+0.011)} &  0.626 \footnotesize{(+0.032)}  &  0.572 \footnotesize{(+0.010)}  &  0.716 \footnotesize{(-0.007)} & 0.426 \footnotesize{(+0.040)} & 0.403 \footnotesize{(+0.031)} & 0.412 \footnotesize{(+0.085)} \\
            \rowcolor{NavyBlue!10}\model (LLaMA3, $k = 1$) & 0.687 \footnotesize{(-0.016)}  & 0.628 \footnotesize{(+0.018)}  &  \textbf{\textcolor{NavyBlue}{0.578}} \footnotesize{\textcolor{NavyBlue}{(+0.016)}}  &  0.730 \footnotesize{(-0.014)}  & 0.465 \footnotesize{(-0.008)}  & 0.430 \footnotesize{(+0.026)} & 0.428 \footnotesize{(+0.033)}   \\
            \rowcolor{NavyBlue!10}\model (LLaMA3, $k = 2$) & 0.682 \footnotesize{(-0.014)}  &  \textbf{\textcolor{NavyBlue}{0.638}} \footnotesize{\textcolor{NavyBlue}{(+0.022)}}  & 0.566 \footnotesize{(-0.000)}  &  \textbf{\textcolor{NavyBlue}{0.736}} \footnotesize{\textcolor{NavyBlue}{(+0.013)}} & \textbf{\textcolor{NavyBlue}{0.527}} \footnotesize{\textcolor{NavyBlue}{(+0.070)}} & \textbf{\textcolor{NavyBlue}{0.463}} \footnotesize{\textcolor{NavyBlue}{(+0.049)}} & \textbf{\textcolor{NavyBlue}{0.489}} \footnotesize{\textcolor{NavyBlue}{(+0.094)}}\\
            \rowcolor{NavyBlue!10}\model (LLaMA3, $k = 3$) & \textbf{\textcolor{NavyBlue}{0.696}} \footnotesize{\textcolor{NavyBlue}{(+0.018)}} &  0.632 \footnotesize{(+0.004)} &   0.572 \footnotesize{(-0.018)}&  0.733 \footnotesize{(-0.004)} & 0.489 \footnotesize{(+0.020)} & 0.411 \footnotesize{(-0.040)}& 0.429 \footnotesize{(+0.018)} \\
            \textbf{\textcolor{NavyBlue}{Improvement over best baseline}} & \textbf{\textcolor{NavyBlue}{+8.8\%}}  &  \textbf{\textcolor{NavyBlue}{+18.0\%}} & \textbf{\textcolor{NavyBlue}{+1.6\%}}  & \textbf{\textcolor{NavyBlue}{+2.2\%}}  & \textbf{\textcolor{NavyBlue}{+18.4\%}} & \textbf{\textcolor{NavyBlue}{+14.9\%}}  & \textbf{\textcolor{NavyBlue}{+16.2\%}}\\ 
            \midrule
            \rowcolor{Red!10}\model (LLaMA3.1, w/o Review) & 0.659 \footnotesize{(-0.036)} &  0.526 \footnotesize{(-0.020)} & 0.556 \footnotesize{(-0.004)}  &  0.726 \footnotesize{(-0.010)} & 0.457 \footnotesize{(+0.159)} & 0.435 \footnotesize{(+0.136)} & 0.439 \footnotesize{(+0.112)} \\
            \rowcolor{Red!10}\model (LLaMA3.1, w/o Revise) & 0.695 \footnotesize{(-0.021)}  &  0.626 \footnotesize{(+0.053)}  &  0.556 \footnotesize{(-0.012)}  &  0.736 \footnotesize{(-0.013)}  & \textbf{\textcolor{Red}{0.489}} \footnotesize{\textcolor{Red}{(+0.097)}}  &  0.436 \footnotesize{(+0.099)} & 0.451 \footnotesize{(+0.099)} \\
            \rowcolor{Red!10}\model (LLaMA3.1, $k = 1$)  &  \textbf{\textcolor{Red}{0.720}} \footnotesize{\textcolor{Red}{(-0.014)}} & \textbf{\textcolor{Red}{0.644}} \footnotesize{\textcolor{Red}{(+0.026)}}  &  0.560 \footnotesize{(-0.059)}  & \textbf{\textcolor{Red}{0.757}} \footnotesize{\textcolor{Red}{(-0.006)}}  & 0.469 \footnotesize{(-0.014)}  & 0.454 \footnotesize{(-0.003)} & 0.437 \footnotesize{(+0.028)} \\
            \rowcolor{Red!10}\model (LLaMA3.1, $k = 2$) & 0.704 \footnotesize{(-0.016)}  & 0.636 \footnotesize{(+0.020)}   &  \textbf{\textcolor{Red}{0.572}} \footnotesize{\textcolor{Red}{(-0.084)}}  & 0.734 \footnotesize{(-0.011)}  & 0.469 \footnotesize{(+0.073)}  & 0.446 \footnotesize{(-0.008)}   & 0.432 \footnotesize{(+0.090)} \\
            \rowcolor{Red!10}\model (LLaMA3.1, $k = 3$) & 0.712 \footnotesize{(-0.004)} &  0.639 \footnotesize{(+0.019)} & 0.562 \footnotesize{(-0.076)}  & 0.748 \footnotesize{(-0.001)} & 0.449 \footnotesize{(-0.020)} & \textbf{\textcolor{Red}{0.470}} \footnotesize{\textcolor{Red}{(+0.059)}} & \textbf{\textcolor{Red}{0.451}} \footnotesize{\textcolor{Red}{(+0.004)}} \\
            \textbf{\textcolor{Red}{Improvement over best baseline}} & \textbf{\textcolor{Red}{+2.4\%}}  & \textbf{\textcolor{Red}{+8.1\%}}  & \textbf{\textcolor{Red}{+0.0\%}}   & \textbf{\textcolor{Red}{+4.9\%}}  & \textbf{\textcolor{Red}{+16.7\%}} & \textbf{\textcolor{Red}{+17.6\%}}  & \textbf{\textcolor{Red}{+11.6\%}}\\ 
            \toprule
	\end{tabular}
 }
\label{open_reasoning_results}
\end{table*}
